Learning Early Exit Strategies for Additive Ranking Ensembles

Modern search engine ranking pipelines are commonly based on large machine-learned ensembles of regression trees. We propose LEAR, a novel - learned - technique aimed to reduce the average number of trees traversed by documents to accumulate the scores, thus reducing the overall query response time. LEAR exploits a classifier that predicts whether a document can early exit the ensemble because it is unlikely to be ranked among the final top-k results. The early exit decision occurs at a sentinel point, i.e., after having evaluated a limited number of trees, and the partial scores are exploited to filter out non-promising documents. We evaluate LEAR by deploying it in a production-like setting, adopting a state-of-the-art algorithm for ensembles traversal. We provide a comprehensive experimental evaluation on two public datasets. The experiments show that LEAR has a significant impact on the efficiency of the query processing without hindering its ranking quality. In detail, on a first dataset, LEAR is able to achieve a speedup of 3x without any loss in NDCG1@0, while on a second dataset the speedup is larger than 5x with a negligible NDCG@10 loss (< 0.05%).

==> 00.ccs.tex <==
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10003317.10003338.10003343</concept_id>
<concept_desc>Information systems~Learning to rank</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002951.10003317.10003359.10003363</concept_id>
<concept_desc>Information systems~Retrieval efficiency</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002951.10003317.10003359.10003362</concept_id>
<concept_desc>Information systems~Retrieval effectiveness</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Learning to rank}
\ccsdesc[500]{Information systems~Retrieval efficiency}
\ccsdesc[500]{Information systems~Retrieval effectiveness}

==> makefile <==
### Makefile for LaTeX under Mac OS X
### Author: Franco Maria Nardini (francomaria.nardini@isti.cnr.it)
# pdflatex, textmate, and skim are needed to run properly all the commands here.

# Some assumptions:
# ./img: is the directory containing images
# ./style: is the directory containing the .cls and .sty

# NAME OF THE MAIN FILE (WITHOUT .tex)
BASEFILENAME=paper

# NAME OF THE BIBLIO FILE (WITHOUT .bib)
BIBLIOFILENAME=biblio

# NAME OF THE CAMERA READY FILE (WITHOUT .pdf)
DESTFILENAME=

# NAME OF THE COVER LETTER FILE (WITHOUT .pdf)
COVERFILENAME=


${BASEFILENAME}.pdf: *.tex ${BASEFILENAME}.aux ${BASEFILENAME}.bbl
	@pdflatex ${BASEFILENAME}.tex
	@open -F -a skim ${BASEFILENAME}.pdf &

${BASEFILENAME}.aux: *.tex
	@pdflatex ${BASEFILENAME}.tex

${BASEFILENAME}.bbl: ${BIBLIOFILENAME}.bib
	@bibtex ${BASEFILENAME}
	@pdflatex ${BASEFILENAME}.tex

all:
	@make clean
	@make pdf
	@make open

pdf:
	@pdflatex ${BASEFILENAME}.tex
	@bibtex ${BASEFILENAME}
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex

open:
	@open -F -a skim ${BASEFILENAME}.pdf

pdf-cameraready:
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex
	@mv ${BASEFILENAME}.pdf ${DESTFILENAME}.pdf
	@open -F -a skim ${DESTFILENAME}.pdf

pdf-coverletter:
	@pdflatex ${COVERFILENAME}.tex
	@bibtex ${BASEFILENAME}
	@pdflatex ${COVERFILENAME}.tex
	@pdflatex ${COVERFILENAME}.tex
	@rm ${COVERFILENAME}.aux
	@rm ${COVERFILENAME}.log
	@open -F -a skim ${COVERFILENAME}.pdf

images:
	@for filename in `ls ./img/*.eps`; do epstopdf $$filename; done;

count:
	@pdftotext ${BASEFILENAME}.pdf WORDS
	@wc --words WORDS
	@rm -f WORDS

clean:
	@rm -f ./img/*~ *~ *spl .*.lb *loa *aux *dvi *maf *mtc *mtc0 *log *fls *lof *lot *out *pdf *bbl *blg *ps *idx *toc *fdb_latexmk *synctex.gz *auxlock *cut

chkrefs:
	@bibtex ${BASEFILENAME}

tgz:
	@tar -czf $(PWD)\ `date +%Y%m%d%H%M`.tar.gz *tex *tmproj *bib ./img/* ./style/*

svn-commit:
	@svn update
	@svn commit -m "`date +%Y%m%d%H%M` - FM"

svn-update:
	@svn update

git-commit-push:
	@git commit -am "`date +%Y%m%d%H%M` - FM"
	@git push origin master

git-pull:
	@git pull origin master


